Seen but Not Connected: Recovering Vessel Trees Below the Threshold

Current segmentation networks reconstruct the distal branches of vessel trees incompletely. To improve completeness, existing methods train the network with topology-aware losses, or track and repair vessels after segmentation. Either way, the network output still passes a fixed threshold, usually 0.5, which ignores true vessels that the map may hold at low probability. A lower threshold keeps them but thickens existing vessels. We propose RIDGER (RIDGE Rooting), which extends the 0.5 mask along the trend of the probability map instead of lowering the threshold. RIDGER first finds vessel ridges in the map, which are the lines of locally highest probability, and keeps the long, confident ridges that join the mask as centrelines. RIDGER then estimates the vessel thickness adaptively: from the 0.5 mask for the proximal vessels and from the probability profile across the vessel for the distal ones. On the other hand, the commonly used metric, Dice, barely drops when the distal vessels are reconstructed incompletely. To indicate the performance of distal vessel reconstruction, we propose a new metric, the reaching rate (R). R is the ratio of the length that the mask covers and connects to the root to the full length of the last 20 mm of each reference branch. When the proposed method, RIDGER, replaces nnU-Net's 0.5 threshold, the metric R rises from 77% to 91% (coronary) and from 80% to 96% (pulmonary), without retraining the network.

==> supp_v2/0_map.tex <==
\providecolor{ridger}{RGB}{252,234,230}\providecolor{subhead}{gray}{0.96}
\makeatletter\@ifundefined{details}{\newenvironment{details}{\par\smallskip\begingroup\footnotesize\def\paragraph##1{\par\smallskip\noindent\textbf{##1} \ignorespaces}\noindent\textbf{Details.}\par\nobreak\noindent\ignorespaces}{\par\endgroup\smallskip}}{}\makeatother
\section*{Overview}
\label{S-sec:supp-0_map}

This appendix gives the method details, the proofs, the protocols and the full results behind the main text. It follows the order of the main text, and each section names the part of the main text that it supports. Paragraphs marked \emph{Details}, in smaller type, hold protocols and secondary analyses. Tables and figures here are numbered S1, S2, and so on; main-text tables keep their numbers.

{\makeatletter\setcounter{tocdepth}{1}\small
\renewcommand*\l@section{\@dottedtocline{1}{0em}{2.3em}}
\renewcommand*\l@subsection{\@dottedtocline{2}{0.9em}{3.0em}}
\def\numberline#1{#1\hskip 1em}%
\tableofcontents\makeatother}
\setcounter{tocdepth}{2}%

